Robustifying Vision-Language Models via Test-Time Prompt Adaptation

Pre-trained Vision-Language Models (VLMs) such as CLIP achieve strong zero-shot generalization, but their performance degrades sharply under adversarial perturbations. Existing test-time adaptation methods typically rely on sample-level confidence heuristics, overlooking the intrinsic distributional structure of the data. This sample-centric approach limits robustness, as it fails to distinguish confident adversarial mispredictions from true semantic consistency. In this work, we observe that adversarial distortion is structurally brittle: while holistic representations are corrupted, semantic integrity is often preserved in the distribution of augmented views. Motivated by this insight, we propose RITA, a Robust test-tIme prompt-TAdaptation framework that shifts from sample-level estimates to distribution-level alignment. Specifically, RITA employs optimal transport to align the distribution of augmented visual features with textual prototypes, mitigating adversarial outliers and rectifying cross-modal semantic misalignment. Furthermore, we introduce a dynamic cache to progressively accumulate reliable cues from the test stream for online refinement. Extensive experiments demonstrate that RITA significantly improves adversarial robustness without compromising clean accuracy.

==> Tables/res_RN50.tex <==
\setlength{\tabcolsep}{4.0pt}
\begin{table*}[ht]
\vspace{-5pt}
  \centering
  \resizebox{0.98\linewidth}{!}{%
  \begin{tabular}{l|ca|ca|ca|ca|ca|ca|ca|ca|ca}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Caltech101} & \multicolumn{2}{c|}{Pets} & \multicolumn{2}{c|}{Cars} & \multicolumn{2}{c|}{Flower102} & \multicolumn{2}{c|}{Aircraft} & \multicolumn{2}{c|}{DTD} & \multicolumn{2}{c|}{EuroSAT} & \multicolumn{2}{c|}{UCF101} & \multicolumn{2}{c}{Avg.} \\
    & Acc. & \multicolumn{1}{c|}{Rob.} & Acc. & \multicolumn{1}{c|}{Rob.} & Acc. & \multicolumn{1}{c|}{Rob.} & Acc. & \multicolumn{1}{c|}{Rob.} & Acc. & \multicolumn{1}{c|}{Rob.} & Acc. & \multicolumn{1}{c|}{Rob.} & Acc. & \multicolumn{1}{c|}{Rob.} & Acc. & \multicolumn{1}{c|}{Rob.} & Acc. & \multicolumn{1}{c}{Rob.} \\
    \midrule

    CLIP \cite{radford2021learning} & 85.9 & 2.6  & 83.5 & 0.0  & 55.7 & 0.0  & 61.7 & 0.0  & 15.7 & 0.0 & 40.4 & 0.8  & 23.7 & 0.0  & 58.9 & 0.0  & 53.2 & 0.4  \\
    Ensemble & 83.5 & 74.8 & 82.3 & 69.9 & 57.1 & 36.2 & 58.0 & 46.6 & 16.4 & 9.8 & 37.1 & 29.5 & 16.7 & 13.7 & 53.9 & 43.0 & 50.6 & 40.4 \\
    TPT \cite{shu2022test} & \bestclean{87.9} & 7.0  & 84.7 & 0.1  & 58.4 & 0.0  & 62.1 & 0.0  & 17.3 & 0.0 & \bestclean{42.4} & 4.3  & \bestclean{28.4} & 0.0  & \bestclean{60.6} & 0.3  & 55.2 & 1.5  \\
    C-TPT \cite{yoon2024c} & 87.7 & 3.7  & 83.6 & 0.0  & 56.6 & 0.0  & \bestclean{64.8} & 0.0  & 16.7 & 0.0 & 41.5 & 1.3  & 27.0 & 0.0  & 60.1 & 0.1  & \bestclean{54.8} & 0.6  \\
    MTA \cite{zanella2024test} & 87.3 & 65.9 & \bestclean{84.8} & 59.8 & \bestclean{58.7} & 17.8 & 61.0 & 31.5 & \bestclean{18.1} & 3.7 & 40.3 & 18.8 & 22.5 & 1.6  & \bestclean{60.6} & 31.3 & 54.1 & 28.8 \\
    R-TPT & 86.7 & \best{79.8} & 84.6 & \best{74.2} & 58.1 & \best{42.9} & 60.6 & \best{51.9} & 17.5 & \best{12.6} & 41.3 & \best{33.5} & 21.2 & \best{15.9} & 59.7 & \best{50.9} & 53.7 & \best{45.2} \\
  
    \bottomrule
  \end{tabular}
}
\caption{Results (\%) of clean accuracy (Acc.) and adversarial accuracy (Rob.) of various adaptation methods on \textbf{fine-grained classification datasets} with pre-trained CLIP-ResNet50 ($\epsilon$ = 1.0). Best clean accuracies are (\bestclean{bold}), best adversarial accuracies are (\best{bold red}).}
\label{tab:fine-grained}
\end{table*}

==> Tables/res_vit16.tex <==
% \setlength{\tabcolsep}{4.0pt}
\begin{table*}[ht]
% \vspace{-5pt}
  \centering
  \tabstyle{3pt}
  \caption{Results (\%) of various adaptation methods on \textbf{fine-grained classification datasets} with pre-trained CLIP-ViT-B/16 ($\epsilon$ = 4.0).
  % \resizebox{0.98\linewidth}{!}{%
  \begin{tabular}{l|ca|ca|ca|ca|ca|ca|ca|ca|ca}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{2}{c|}{Caltech101} & \multicolumn{2}{c|}{Pets} & \multicolumn{2}{c|}{Cars} & \multicolumn{2}{c|}{Flower102} & \multicolumn{2}{c|}{Aircraft} & \multicolumn{2}{c|}{DTD} & \multicolumn{2}{c|}{EuroSAT} & \multicolumn{2}{c|}{UCF101} & \multicolumn{2}{c}{Avg.} \\
    & Acc. & \multicolumn{1}{c|}{Rob.} & Acc. & \multicolumn{1}{c|}{Rob.} & Acc. & \multicolumn{1}{c|}{Rob.} & Acc. & \multicolumn{1}{c|}{Rob.} & Acc. & \multicolumn{1}{c|}{Rob.} & Acc. & \multicolumn{1}{c|}{Rob.} & Acc. & \multicolumn{1}{c|}{Rob.} & Acc. & \multicolumn{1}{c|}{Rob.} & Acc. & \multicolumn{1}{c}{Rob.} \\
    \midrule
    CLIP \cite{radford2021learning} & 94.0 & 0.0  & \bestclean{88.3} & 0.0  & 65.5 & 0.0  & 67.4 & 0.0  & 23.9 & 0.0 & 44.4 & 0.0  & 42.2 & 0.0 & 65.2 & 0.0  & 61.4 & 0.0 \\
    Ensemble & 91.9 & 74.7 & 86.2 & 51.2 & 65.7 & 26.0 & 65.9 & 36.3 & 23.4 & 8.7 & 43.2 & 25.1 & 28.2 & 2.2 & 63.0 & 30.6 & 58.4 & 31.8 \\
    TPT \cite{shu2022test} & 94.1 & 0.0  & 87.4 & 0.0  & 66.5 & 0.0  & 69.1 & 0.0  & 23.4 & 0.0 & \bestclean{46.9} & 0.0  & \bestclean{42.6} & 0.0 & \bestclean{67.9} & 0.0  & 62.2 & 0.0  \\
    C-TPT \cite{yoon2024c} & 93.9 & 0.0  & 88.2 & 0.0  & 65.8 & 0.0  & \bestclean{69.6} & 0.0  & 23.9 & 0.0 & 45.9 & 0.0  & 42.3 & 0.0 & 65.5 & 0.0  & 61.9 & 0.0  \\
    MTA \cite{zanella2024test} & \bestclean{94.3} & 72.1 & 88.0 & 51.8 & \bestclean{67.7} & 18.5 & 67.4 & 27.9 & \bestclean{25.0} & 4.3 & 46.5 & 16.2 & 42.5 & 1.2 & 67.5 & 27.5 & \bestclean{62.3} & 27.4 \\
    R-TPT  & 93.7 & \best{82.0} & 87.2 & \best{60.2} & 67.0 & \best{34.7} & 68.7 & \best{44.6} & 23.9 & \best{13.2} & 46.4 & \best{32.8} & 34.7 & \best{8.5} & 67.2 & \best{43.2} & 61.1 & \best{39.9} \\
    \ours  & 93.7 & \best{82.0} & 87.2 & \best{60.2} & 67.0 & \best{34.7} & 68.7 & \best{44.6} & 23.9 & \best{13.2} & 46.4 & \best{32.8} & 34.7 & \best{8.5} & 67.2 & \best{43.2} & 61.1 & \best{39.9} \\
    \bottomrule
  \end{tabular}
}
% }
\label{tab:vitb16}
\end{table*}
